BoolGebra: Attributed Graph-learning for Boolean Algebraic Manipulation

Boolean algebraic manipulation is at the core of logic synthesis in Electronic Design Automation (EDA) design flow. Existing methods struggle to fully exploit optimization opportunities, and often suffer from an explosive search space and limited scalability efficiency. This work presents BoolGebra, a novel attributed graph-learning approach for Boolean algebraic manipulation that aims to improve fundamental logic synthesis. BoolGebra incorporates Graph Neural Networks (GNNs) and takes initial feature embeddings from both structural and functional information as inputs. A fully connected neural network is employed as the predictor for direct optimization result predictions, significantly reducing the search space and efficiently locating the optimization space. The experiments involve training the BoolGebra model w.r.t design-specific and cross-design inferences using the trained model, where BoolGebra demonstrates generalizability for cross-design inference and its potential to scale from small, simple training datasets to large, complex inference datasets. Finally, BoolGebra is integrated with existing synthesis tool ABC to perform end-to-end logic minimization evaluation w.r.t SOTA baselines.

==> alg_local.tex <==
\begin{algorithm}
\caption{DAG-aware local greedy orchestration}   
\label{alg:local}
 
   \SetKwInOut{KwIn}{Input}
    \SetKwInOut{KwOut}{Output}
    \KwIn{~$G(V,E) \leftarrow$ Boolean Networks/Circuits in AIG} 
    \KwOut{~Post-optimized AIG $G(V,E)$}
 \For{$v \in V$ in topological order}{
 %\tcp{New order}
       check transformability of $v$ w.r.t orchestrated operations: \texttt{rw}, \texttt{rs}, \texttt{rf}, and get the corresponding optimization gain: \texttt{G$_{rw}^{v}$}, \texttt{G$_{rs}^{v}$}, \texttt{G$_{rf}^{v}$}.
        \tcp*[f]{if operation is not applicable, $G$ is $-1$; otherwise, $G$ is a non-negative number}

  \uIf{\texttt{G$_{rw}^{v}$} $\geq$ 0 and \texttt{G$_{rw}^{v}$} $\geq$ \texttt{G$_{rs}^{v}$} and \texttt{G$_{rw}^{v}$} $\geq$ \texttt{G$_{rf}^{v}$} }{
        $ G(V,E) \xleftarrow{rw} G(V,E)$
        
        continue
     \tcp*[f]{\texttt{rw} with the highest gain}
         }
  \uElseIf{\texttt{G$_{rs}^{v}$} $\geq$ 0 and \texttt{G$_{rs}^{v}$} $\geq$ \texttt{G$_{rw}^{v}$} and \texttt{G$_{rs}^{v}$} $\geq$ \texttt{G$_{rf}^{v}$} }{
            $ G(V,E) \xleftarrow{rs} G(V,E)$
        
        continue
     \tcp*[f]{\texttt{rs} with the highest gain}
  }
  \uElseIf{\texttt{G$_{rf}^{v}$} $\geq$ 0 and \texttt{G$_{rf}^{v}$} $\geq$ \texttt{G$_{rw}^{v}$} and \texttt{G$_{rf}^{v}$} $\geq$ \texttt{G$_{rs}^{v}$} }{
            $ G(V,E) \xleftarrow{rf} G(V,E)$
        
        continue
     \tcp*[f]{\texttt{rf} with the highest gain}
  }
  \Else{
    continue 
  }
  Update $G(V,E) \leftarrow$ \texttt{Dec\_GraphUpdateNetwork}, and exclude $v$ and transformed nodes from $V$
  }

\end{algorithm}

==> figs/analysis_figure.tex <==

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figs/plot_ops_all_s38584.pdf}
        \caption{s38584}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figs/plot_ops_all_s35932.pdf}
        \caption{s35932}
    \end{subfigure}
    \hfill
    %\begin{subfigure}[b]{0.19\textwidth}
    %    \centering
    %    \includegraphics[width=1\textwidth]{figs/plot_ops_all_b17.pdf}
    %    \caption{b17\_1}
    %\end{subfigure}
    %\hfill
    %\begin{subfigure}[b]{0.19\textwidth}
    %    \centering
    %    \includegraphics[width=1\textwidth]{figs/plot_ops_all_b18.pdf}
    %    \caption{b18\_1}
    %\end{subfigure}
    %\hfill
    %\begin{subfigure}[b]{0.19\textwidth}
    %    \centering
    %    \includegraphics[width=1\textwidth]{figs/plot_ops_all_b21.pdf}
    %    \caption{b21}
    %\end{subfigure}
    %\hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figs/plot_ops_all_bfly.pdf}
        \caption{bfly}
        \label{fig:ana_bfly}
    \end{subfigure}
    \hfill
    %\begin{subfigure}[b]{0.2\textwidth}
    %    \centering
    %    \includegraphics[width=1\textwidth]{figs/plot_ops_all_fir.pdf}
    %    \caption{fir}
    %\end{subfigure}
    %\hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{figs/plot_ops_all_mem_ctrl.pdf}
        \caption{mem\_ctrl}
    \end{subfigure}
    %\hfill
    %\begin{subfigure}[b]{0.19\textwidth}
    %    \centering
    %    \includegraphics[width=1\textwidth]{figs/plot_ops_all_sqrt.pdf}
    %    \caption{sqrt}
    %\end{subfigure}
    %\hfill
    %\begin{subfigure}[b]{0.19\textwidth}
    %    \centering
    %    \includegraphics[width=1\textwidth]{figs/plot_ops_all_voter.pdf}
    %    \caption{voter}
    %    \label{fig:ana_voter}
    %\end{subfigure}
     \caption{The optimization space (node size) with different optimization operations. The $X-$axis denotes the operations for AIG optimization. The $Y-$axis denotes the number of nodes applicable to the corresponding operation.}
    % \vspace{-2mm}
     \label{fig:ana}
\end{figure}


==> figs/results_1o_plot.tex <==

\begin{figure}[!htb]
\begin{subfigure}[b]{0.49\linewidth}
  \centering
  % include first image
  \includegraphics[width=1\linewidth]{1Oplot/1_O_O1.pdf}  
  \caption{\texttt{rw/rs/rf} vs. $\widehat{\texttt{O1}}$}
  \label{fig:1O_O1}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.49\linewidth}
  \centering
  % include second image
  \includegraphics[width=1\linewidth]{1Oplot/1_O_O2.pdf}  
  \caption{\texttt{rw/rs/rf} vs. $\widehat{\texttt{O2}}$}
  \label{fig:1O_O2}
\end{subfigure}
\hfill

\begin{subfigure}{0.49\linewidth}
  \centering
  % include third image
  \includegraphics[width=1\linewidth]{1Oplot/1_O_O3.pdf}  
  \caption{\texttt{rw/rs/rf} vs. $\widehat{\texttt{O3}}$}
  \label{fig:1O_O3}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\linewidth}
  \centering
  % include fourth image
  \includegraphics[width=1\linewidth]{1Oplot/1_O_O4.pdf}  
  \caption{\texttt{rw/rs/rf} vs. $\widehat{\texttt{O4}}$}
  \label{fig:1O_O4}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\linewidth}
  \centering
  % include fifth image
  \includegraphics[width=1\linewidth]{1Oplot/1_O_O5.pdf}  
  \caption{\texttt{rw/rs/rf} vs. $\widehat{\texttt{O5}}$}
  \label{fig:1O_O5}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\linewidth}
  \centering
  % include sixth image
  \includegraphics[width=1\linewidth]{1Oplot/1_O_O6.pdf}  
  \caption{\texttt{rw/rs/rf} vs. $\widehat{\texttt{O6}}$}
  \label{fig:1O_O6}
\end{subfigure}
\caption{Normalized node number comparison of the same design after applying stand-alone optimizations and \texttt{orchestration} with a single AIG traversal. \textbf{R} is the ratio of the number of designs on which \texttt{orchestration} outperforms stand-alone optimization to the number of total tested designs.}
\vspace{-4mm}
\label{fig:1O}
\end{figure}


==> figs/results_3o_plot.tex <==
\begin{figure}[!htb]
\centering
\begin{subfigure}[b]{0.49\linewidth}
  \centering
  % include first image
  \includegraphics[width=1.\linewidth]{3Oplot/3_O_1.pdf}  
  \caption{Seq(ABC) vs. Seq($\widehat{\texttt{O1}}$)}
  \label{fig:3O_O1}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\linewidth}
  \centering
  % include third image
  \includegraphics[width=1.\linewidth]{3Oplot/3_O_3.pdf}  
  \caption{Seq(ABC) vs. Seq($\widehat{\texttt{O3}}$)}
  \label{fig:3O_O3}
\end{subfigure}

\caption{Normalized node number comparison between iterative \texttt{orchestration} and iterative ABC SOTA optimizations. \textbf{R} is the ratio of the number of designs on which Seq($\widehat{\texttt{On}}$) outperforms Seq(ABC) to the number of total tested designs.}
%\vspace{-3mm}
\label{fig:3O}
\end{figure}


\iffalse

\begin{figure}[!htb]
\begin{subfigure}[b]{0.49\linewidth}
  \centering
  % include first image
  \includegraphics[width=1.\linewidth]{3Oplot/3_O_1.pdf}  
  \caption{Seq(ABC) vs. Seq($\widehat{O1}$)}
  \label{fig:3O_O1}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.49\linewidth}
  \centering
  % include second image
  \includegraphics[width=1.\linewidth]{3Oplot/3_O_2.pdf}  
  \caption{Seq(ABC) vs. Seq($\widehat{O2}$)}
  \label{fig:3O_O2}
\end{subfigure}
\hfill

\begin{subfigure}{0.49\linewidth}
  \centering
  % include third image
  \includegraphics[width=1.\linewidth]{3Oplot/3_O_3.pdf}  
  \caption{Seq(ABC) vs. Seq($\widehat{O3}$)}
  \label{fig:3O_O3}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\linewidth}
  \centering
  % include fourth image
  \includegraphics[width=1.\linewidth]{3Oplot/3_O_4.pdf}  
  \caption{Seq(ABC) vs. Seq($\widehat{O4}$)}
  \label{fig:3O_O4}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\linewidth}
  \centering
  % include fifth image
  \includegraphics[width=1.\linewidth]{3Oplot/3_O_5.pdf}  
  \caption{Seq(ABC) vs. Seq($\widehat{O5}$)}
  \label{fig:3O_O5}
\end{subfigure}
\hfill
\begin{subfigure}{0.49\linewidth}
  \centering
  % include sixth image
  \includegraphics[width=1.\linewidth]{3Oplot/3_O_6.pdf}  
  \caption{Seq(ABC) vs. Seq($\widehat{O6}$)}
  \label{fig:3O_O6}
\end{subfigure}

\caption{Normalized node number comparison between iterative orchestrations and iterative ABC SOTA optimizations. \texttt{R} is the ratio of number of designs where our orchestration outperforms ABC sequences.}
\vspace{-3mm}
\label{fig:3O}
\end{figure}
\fi

==> tbls/tabel_end-to-end.tex <==
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
 &    &   &   & &  &  &  &  &      \\
\multirow{-2}{*}{} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Logic Synthesis \\ (resyn)\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Logic Synthesis\\ (LGP-resyn)\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Logic Synthesis\\  (O-resyn)\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Tech Map\\  (resyn)\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Tech Map\\ (LGP-resyn)\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Tech Map\\  (O-resyn)\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Post-routing \\ (resyn)\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Post-routing\\ (LGP-resyn)\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Post-routing\\ (O-resyn)\end{tabular}} \\ \hline
   & Node   & Node   & Node  & Area      & Area & Area    & Area/$um^{2}$       & Area/$um^{2}$       & Area/$um^{2}$        \\ \hline
s38584             & 10391                                                                                & 10121 (-2.6\%)                                                                             & 10059 (-3.2\%)                                                                                & 13161.95                                                                      & 13000.48 (-1.2\%)                                                                   & 13011.922 (-1.1\%)                                                                     & 14313                                                                             & 14013 (-2.1\%)                                                                          & 14137 (-1.2\%)                                                                            \\ \hline
s35932             & 8518   & 8113 (-4.8\%)    & 8113 (-4.8\%)                                                         & 15368.15                                              & 15372.40 (+0.03\%)              &15368.15 (0)   & 16045      & 16055 (+0.06\%)        & 16045 (0)                                                         \\ \hline
b17\_1             & 23021                                                                                & 22043 (-4.2\%)                                                                             & 21603 (-6.2\%)                                                                                & 26798.44                                                                      & 25640.27 (-4.3\%)                                                                                    & 26019.588 (-2.9\%)                                                                     & 29138                                                                             &   28193 (-3.2\%)                                                                                      & 28561 (-2.0\%)                                                                            \\ \hline
b18\_1             & 63151                                                                                & 60215 (-4.6\%)                                                                             & 59336 (-6.0\%)                                                                                & 70259.38                                                                      & 68211.18 (-2.9\%)                                                                   & 67852.876 (-3.4\%)                                                                     & 76811                                                                             & 74499 (-3.0\%)                                                                          & 74516 (-3.0\%)                                                                            \\ \hline
b20                & 10152                                                                                & 9715 (-4.3\%)                                                                              & 9610 (-5.3\%)                                                                                 & 11295.96                                                                      & 10915.57 (-3.3\%)                                                                   & 11029.158 (-2.4\%)                                                                     & 12247                                                                             & 11861 (-3.1\%)                                                                          & 12027 (-1.8\%)                                                                            \\ \hline
b21                & 10211                                                                                & 9806 (-4.0\%)                                                                              & 9736 (-4.6\%)                                                                                 & 11585.63                                                                      & 11190.09 (-3.4\%)                                                                   & 11222.274 (-3.1\%)                                                                     & 12596                                                                             & 12246 (-2.7\%)                                                                          & 12276 (-2.5\%)                                                                            \\ \hline
b22                & 15067                                                                                & 14506 (-3.7\%)                                                                             & 14404 (-4.4\%)                                                                                & 16115.61                                                                      & 15879.67 (-1.4\%)                                                                   & 15928.612 (-1.2\%)                                                                     & 17856                                                                             & 17404 (-2.5\%)                                                                          & 17518 (-1.9\%)                                                                            \\ \hline
\end{tabular}
}
\caption{The results reported by OpenROAD with orchestration methods implementation, including the results from logic synthesis, i.e., AIG minimization, technology mapping with nangate 45nm, and post-routing.}
\label{tbl:resyn_openroad}
\end{table*}





==> tbls/table_1o.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|ccccccccccccc|}
\hline
\multicolumn{2}{|c|}{\multirow{3}{*}{Design}} & \multicolumn{11}{c|}{AIG} \\ \cline{3-13} 
\multicolumn{2}{|c|}{} & \multicolumn{1}{c|}{Baseline} & \multicolumn{1}{c|}{\texttt{rw}} & \multicolumn{1}{c|}{\texttt{rs}} & \multicolumn{1}{c|}{\texttt{rf}} & \multicolumn{1}{c|}{$\widehat{\texttt{O1}}$} & \multicolumn{1}{c|}{$\widehat{\texttt{O2}}$} & \multicolumn{1}{c|}{$\widehat{\texttt{O3}}$} & \multicolumn{1}{c|}{$\widehat{\texttt{O4}}$} & \multicolumn{1}{c|}{$\widehat{\texttt{O5}}$} & \multicolumn{1}{c|}{$\widehat{\texttt{O6}}$} & ${\texttt{LocalGreedy}}$\\ \cline{3-13} 
\multicolumn{2}{|c|}{} & \multicolumn{1}{c|}{\#Node} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \#Node ($\Delta$\%) \\ \hline
\multicolumn{1}{|c|}{\multirow{7}{*}{ISCAS}} & \multicolumn{1}{c|}{s38584} & \multicolumn{1}{c|}{12400} & \multicolumn{1}{c|}{10697 (13.7\%)} & \multicolumn{1}{c|}{11505 (7.2\%)} & \multicolumn{1}{c|}{10932 (11.8\%)} & \multicolumn{1}{c|}{10366 (16.4\%)} & \multicolumn{1}{c|}{10379 (16.3\%)} & \multicolumn{1}{c|}{\textbf{10336 (16.7\%)}} & \multicolumn{1}{c|}{10655 (14.1\%)} & \multicolumn{1}{c|}{10932 (11.8\%)} & \multicolumn{1}{c|}{10932 (11.8\%)} & 10449 (15.7\%) \\ \cline{2-13} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{s35932} & \multicolumn{1}{c|}{11948} & \multicolumn{1}{c|}{9110 (23.8\%)} & \multicolumn{1}{c|}{11916 (0.3\%)} & \multicolumn{1}{c|}{9836 (17.7\%)} & \multicolumn{1}{c|}{\textbf{8561 (28.4\%)}} & \multicolumn{1}{c|}{\textbf{8561 (28.4\%)}} & \multicolumn{1}{c|}{\textbf{8561 (28.4\%)}} & \multicolumn{1}{c|}{9836 (17.7\%)} & \multicolumn{1}{c|}{9836 (17.7\%)} & \multicolumn{1}{c|}{9836 (17.7\%)} & \textbf{8561 (28.4\%)} \\ \cline{2-13} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b17\_1} & \multicolumn{1}{c|}{27647} & \multicolumn{1}{c|}{24178 (12.6\%)} & \multicolumn{1}{c|}{26305 (4.9\%)} & \multicolumn{1}{c|}{24533 (11.3\%)} & \multicolumn{1}{c|}{22951 (17.0\%)} & \multicolumn{1}{c|}{23125 (16.4\%)} & \multicolumn{1}{c|}{\textbf{22935 (17.0\%)}} & \multicolumn{1}{c|}{23393 (15.4\%)} & \multicolumn{1}{c|}{24532 (11.3\%)} & \multicolumn{1}{c|}{24532 (11.3\%)} & {23008 (16.7\%)} \\ \cline{2-13} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b18\_1} & \multicolumn{1}{c|}{79054} & \multicolumn{1}{c|}{66807 (15.5\%)} & \multicolumn{1}{c|}{73076 (7.6\%)} & \multicolumn{1}{c|}{69606 (12.0\%)} & \multicolumn{1}{c|}{63431 (19.8\%)} & \multicolumn{1}{c|}{64135 (18.9\%)} & \multicolumn{1}{c|}{\textbf{63167 (20.1\%)}} & \multicolumn{1}{c|}{65956 (16.6\%)} & \multicolumn{1}{c|}{69586 (12.0\%)} & \multicolumn{1}{c|}{69587 (12.0\%)} & 63726 (19.4\%) \\ \cline{2-13} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b20} & \multicolumn{1}{c|}{12219} & \multicolumn{1}{c|}{10659 (12.8\%)} & \multicolumn{1}{c|}{11197 (8.4\%)} & \multicolumn{1}{c|}{10593 (13.3\%)} & \multicolumn{1}{c|}{10017 (18.02\%)} & \multicolumn{1}{c|}{10110 (17.3\%)} & \multicolumn{1}{c|}{\textbf{10011 (18.1\%)}} & \multicolumn{1}{c|}{10228 (16.3\%)} & \multicolumn{1}{c|}{10590 (13.3\%)} & \multicolumn{1}{c|}{10590 (13.3\%)} & 10129 (17.1\%) \\ \cline{2-13} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b21} & \multicolumn{1}{c|}{12782} & \multicolumn{1}{c|}{10863 (15.1\%)} & \multicolumn{1}{c|}{11449 (10.4\%)} & \multicolumn{1}{c|}{10961 (14.3\%)} & \multicolumn{1}{c|}{10146 (20.6\%)} & \multicolumn{1}{c|}{10237 (19.9\%)} & \multicolumn{1}{c|}{\textbf{10133 (20.7\%)}} & \multicolumn{1}{c|}{10458 (18.2\%)} & \multicolumn{1}{c|}{10958 (14.3\%)} & \multicolumn{1}{c|}{10958 (14.3\%)} & 10261 (19.7\%) \\ \cline{2-13} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b22} & \multicolumn{1}{c|}{18488} & \multicolumn{1}{c|}{15983 (13.6\%)} & \multicolumn{1}{c|}{16891 (8.6\%)} & \multicolumn{1}{c|}{15983 (13.6\%)} & \multicolumn{1}{c|}{14977 (19.0\%)} & \multicolumn{1}{c|}{15115 (18.2\%)} & \multicolumn{1}{c|}{\textbf{14953 (19.1\%)}} & \multicolumn{1}{c|}{15275 (17.4\%)} & \multicolumn{1}{c|}{15965 (13.6\%)} & \multicolumn{1}{c|}{15965 (13.6\%)} & 15127 (18.2\%) \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{VTR}} & \multicolumn{1}{c|}{bfly} & \multicolumn{1}{c|}{28910} & \multicolumn{1}{c|}{26827 (7.2\%)} & \multicolumn{1}{c|}{27060 (6.4\%)} & \multicolumn{1}{c|}{27487 (4.9\%)} & \multicolumn{1}{c|}{\textbf{25996 (10.1\%)}} & \multicolumn{1}{c|}{26183 (9.4\%)} & \multicolumn{1}{c|}{26027 (10.0\%)} & \multicolumn{1}{c|}{26353 (8.8\%)} & \multicolumn{1}{c|}{27487 (4.9\%)} & \multicolumn{1}{c|}{27487 (4.9\%)} & 26181 (9.4\%) \\ \cline{2-13} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{dscg} & \multicolumn{1}{c|}{28252} & \multicolumn{1}{c|}{26132 (7.5\%)} & \multicolumn{1}{c|}{26352 (6.73\%)} & \multicolumn{1}{c|}{26972 (4.5\%)} & \multicolumn{1}{c|}{\textbf{25339 (10.3\%)}} & \multicolumn{1}{c|}{25552 (9.5\%)} & \multicolumn{1}{c|}{25345 (10.3\%)} & \multicolumn{1}{c|}{25768 (8.8\%)} & \multicolumn{1}{c|}{26970 (4.5\%)} & \multicolumn{1}{c|}{26970 (4.5\%)} & {25496 (9.7\%)} \\ \cline{2-13} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{fir} & \multicolumn{1}{c|}{27704} & \multicolumn{1}{c|}{25641 (7.5\%)} & \multicolumn{1}{c|}{25768 (7.0\%)} & \multicolumn{1}{c|}{26437 (4.6\%)} & \multicolumn{1}{c|}{\textbf{24778 (10.6\%)}} & \multicolumn{1}{c|}{25061 (9.5\%)} & \multicolumn{1}{c|}{24831 (10.4\%)} & \multicolumn{1}{c|}{25189 (9.1\%)} & \multicolumn{1}{c|}{26437 (4.6\%)} & \multicolumn{1}{c|}{26437 (4.6\%)} & 24987 (9.8\%) \\ \cline{2-13}

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{syn2} & \multicolumn{1}{c|}{30003} & \multicolumn{1}{c|}{27787 (7.4\%)} & \multicolumn{1}{c|}{28031 (6.6\%)} & \multicolumn{1}{c|}{28617 (4.6\%)} & \multicolumn{1}{c|}{\textbf{27013 (10.0\%)}} & \multicolumn{1}{c|}{27266 (9.1\%)} & \multicolumn{1}{c|}{27048 (9.9\%)} & \multicolumn{1}{c|}{27444 (8.5\%)} & \multicolumn{1}{c|}{28617 (4.6\%)} & \multicolumn{1}{c|}{28617 (4.6\%)} & {27198 (9.3\%)} \\ \hline


\multicolumn{1}{|c|}{\multirow{5}{*}{EPFL}} & \multicolumn{1}{c|}{div} & \multicolumn{1}{c|}{57247} & \multicolumn{1}{c|}{41153 (28.1\%)} & \multicolumn{1}{c|}{52621 (8.1\%)} & \multicolumn{1}{c|}{56745 (0.9\%)} & \multicolumn{1}{c|}{\textbf{41123 (28.2\%)}} & \multicolumn{1}{c|}{41143 (28.1\%)} & \multicolumn{1}{c|}{41124 (28.2\%)} & \multicolumn{1}{c|}{52098 (9.0\%)} & \multicolumn{1}{c|}{56738 (0.9\%)} & \multicolumn{1}{c|}{56738 (0.9\%)} & 41147 (28.1\%) \\ \cline{2-13} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{hyp} & \multicolumn{1}{c|}{214335} & \multicolumn{1}{c|}{214274 (0.0\%)} & \multicolumn{1}{c|}{209164 (2.4\%)} & \multicolumn{1}{c|}{212341 (1.0\%)} & \multicolumn{1}{c|}{207335 (3.3\%)} & \multicolumn{1}{c|}{212327 (0.9\%)} & \multicolumn{1}{c|}{\textbf{207315 (3.3\%)}} & \multicolumn{1}{c|}{\textbf{207315 (3.3\%)}} & \multicolumn{1}{c|}{212338 (1.0\%)} & \multicolumn{1}{c|}{212338 (1.0\%)} & 207319 (3.3\%) \\ \cline{2-13} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{mem\_ctrl} & \multicolumn{1}{c|}{46836} & \multicolumn{1}{c|}{46732 (0.2\%)} & \multicolumn{1}{c|}{46554 (0.6\%)} & \multicolumn{1}{c|}{46574 (0.6\%)} & \multicolumn{1}{c|}{46301 (1.1\%)} & \multicolumn{1}{c|}{46484 (0.8\%)} & \multicolumn{1}{c|}{\textbf{46085 (1.6\%)}} & \multicolumn{1}{c|}{46204 (1.4\%)} & \multicolumn{1}{c|}{46569 (0.6\%)} & \multicolumn{1}{c|}{46569 (0.6\%)} & {46201 (1.3\%)} \\ \cline{2-13}

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{sqrt} & \multicolumn{1}{c|}{24618} & \multicolumn{1}{c|}{19441 (21.0\%)} & \multicolumn{1}{c|}{21690 (11.9\%)} & \multicolumn{1}{c|}{23685 (3.8\%)} & \multicolumn{1}{c|}{\textbf{19221 (21.9\%)}} & \multicolumn{1}{c|}{19441 (21.0\%)} & \multicolumn{1}{c|}{\textbf{19221 (21.9\%)}} & \multicolumn{1}{c|}{21582 (12.3\%)} & \multicolumn{1}{c|}{23685 (3.8\%)} & \multicolumn{1}{c|}{23685 (3.8\%)} & 19221 (21.9\%) \\ \cline{2-13} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{voter} & \multicolumn{1}{c|}{13758} & \multicolumn{1}{c|}{11408 (17.0\%)} & \multicolumn{1}{c|}{10997 (20.1\%)} & \multicolumn{1}{c|}{12681 (7.8\%)} & \multicolumn{1}{c|}{9461 (31.2\%)} & \multicolumn{1}{c|}{10982 (20.2\%)} & \multicolumn{1}{c|}{\textbf{9399 (31.7\%)}} & \multicolumn{1}{c|}{9492 (31.0\%)} & \multicolumn{1}{c|}{12679 (7.8\%)} & \multicolumn{1}{c|}{12679 (7.8\%)} & 9606 (30.2\%) \\ \hline
\multicolumn{3}{|c|}{\textbf{Avg. Node Reduction\%}} & \multicolumn{1}{c|}{12.7\%} & \multicolumn{1}{c|}{7.3\%} & \multicolumn{1}{c|}{7.9\%} & \multicolumn{1}{c|}{16.6\%} & \multicolumn{1}{c|}{15.3\%} & \multicolumn{1}{c|}{\textbf{16.7\%}} & \multicolumn{1}{c|}{13.0\%} & \multicolumn{1}{c|}{7.9\%} & \multicolumn{1}{c|}{7.9\%} & 16.1\% \\ \hline
\end{tabular}
}
\caption{Detailed results of selected large size designs. Comparison of single-traversal \texttt{orchestration} with stand-alone optimizations from ABC.}
\vspace{-3mm}
\label{table:1O}
\end{table*}

==> tbls/table_resyn.tex <==
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
% \subfloat[First caption]{%
% \centering

\begin{tabular}{|cccccccccccccccc|}
\hline
\multicolumn{2}{|c|}{\multirow{3}{*}{Design}} & \multicolumn{14}{c|}{AIG: \texttt{resyn}} \\ \cline{3-16} 
\multicolumn{2}{|c|}{} & \multicolumn{2}{c|}{Baseline} & \multicolumn{2}{c|}{\texttt{resyn}} & \multicolumn{2}{c|}{\texttt{resyn3}} & \multicolumn{2}{c|}{$\widehat{\texttt{O}}$\texttt{-resyn}} & \multicolumn{2}{c|}{$\widehat{\texttt{O}}$\texttt{-resyn3}} & \multicolumn{2}{c|}{${\texttt{LGP}}$\texttt{-resyn}} & \multicolumn{2}{c|}{${\texttt{LGP}}$\texttt{-resyn3}} \\ \cline{3-16} 
\multicolumn{2}{|c|}{} & \multicolumn{1}{c|}{\#Node} & \multicolumn{1}{c|}{\#Level} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Level} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Level} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Level} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Level} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Level} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \#Level \\ \hline
\multicolumn{1}{|c|}{\multirow{7}{*}{ISCAS}} & \multicolumn{1}{c|}{s38584} & \multicolumn{1}{c|}{12400} & \multicolumn{1}{c|}{36} & \multicolumn{1}{c|}{10391  (16.2\%)} & \multicolumn{1}{c|}{{25}} & \multicolumn{1}{c|}{11378  (8.2\%)} & \multicolumn{1}{c|}{28} & \multicolumn{1}{c|}{10069  (18.8\%)} & \multicolumn{1}{c|}{\textbf{24}} & \multicolumn{1}{c|}{{10078  (18.7\%)}} & \multicolumn{1}{c|}{{26}} & \multicolumn{1}{c|}{10121  (18.4\%)} & \multicolumn{1}{c|}{{26}} & \multicolumn{1}{c|}{\textbf{10067  (18.8\%)}} & \textbf{24} \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{s35932} & \multicolumn{1}{c|}{11948} & \multicolumn{1}{c|}{19} & \multicolumn{1}{c|}{8518  (28.7\%)} & \multicolumn{1}{c|}{12} & \multicolumn{1}{c|}{11916  (0.3\%)} & \multicolumn{1}{c|}{19} & \multicolumn{1}{c|}{\textbf{8113  (32.1\%)}} & \multicolumn{1}{c|}{\textbf{11}} & \multicolumn{1}{c|}{8177  (31.6\%)} & \multicolumn{1}{c|}{13} & \multicolumn{1}{c|}{\textbf{8113  (32.1\%)}} & \multicolumn{1}{c|}{\textbf{11}} & \multicolumn{1}{c|}{\textbf{8113  (32.1\%)}} & \textbf{11} \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b17\_1} & \multicolumn{1}{c|}{27647} & \multicolumn{1}{c|}{52} & \multicolumn{1}{c|}{23021  (16.7\%)} & \multicolumn{1}{c|}{\textbf{46}} & \multicolumn{1}{c|}{26067  (5.7\%)} & \multicolumn{1}{c|}{47} & \multicolumn{1}{c|}{\textbf{21689  (21.6\%)}} & \multicolumn{1}{c|}{\textbf{46}} & \multicolumn{1}{c|}{{21991  (20.5\%)}} & \multicolumn{1}{c|}{47} & \multicolumn{1}{c|}{22043  (20.2\%)} & \multicolumn{1}{c|}{47} & \multicolumn{1}{c|}{21943  (20.6\%)} & 47 \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b18\_1} & \multicolumn{1}{c|}{79054} & \multicolumn{1}{c|}{132} & \multicolumn{1}{c|}{63151 (20.1\%)} & \multicolumn{1}{c|}{\textbf{114}} & \multicolumn{1}{c|}{70808  (10.4\%)} & \multicolumn{1}{c|}{128} & \multicolumn{1}{c|}{59846  (24.3\%)} & \multicolumn{1}{c|}{121} & \multicolumn{1}{c|}{60084  (24.0\%)} & \multicolumn{1}{c|}{131} & \multicolumn{1}{c|}{60215  (23.8\%)} & \multicolumn{1}{c|}{128} & \multicolumn{1}{c|}{\textbf{59791  (24.4\%)}} & 128 \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b20} & \multicolumn{1}{c|}{12219} & \multicolumn{1}{c|}{66} & \multicolumn{1}{c|}{10152 (16.9\%)} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{11013  (9.9\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{9676  (20.8\%)} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{9627  (21.2\%)} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{9715  (20.5\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{\textbf{9604  (21.4\%)}} & 65 \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b21} & \multicolumn{1}{c|}{12782} & \multicolumn{1}{c|}{67} & \multicolumn{1}{c|}{10211  (20.1\%)} & \multicolumn{1}{c|}{64} & \multicolumn{1}{c|}{11249  (12.0\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{9779  (23.5\%)} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{9725  (23.9\%)} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{9806  (23.3\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{\textbf{9703  (24.1\%)}} & 65 \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b22} & \multicolumn{1}{c|}{18488} & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{15067  (18.5\%)} & \multicolumn{1}{c|}{\textbf{65}} & \multicolumn{1}{c|}{16643  (10.0\%)} & \multicolumn{1}{c|}{\textbf{65}} & \multicolumn{1}{c|}{14525  (21.4\%)} & \multicolumn{1}{c|}{\textbf{65}} & \multicolumn{1}{c|}{14399  (22.1\%)} & \multicolumn{1}{c|}{\textbf{65}} & \multicolumn{1}{c|}{14506  (21.5\%)} & \multicolumn{1}{c|}{\textbf{65}} & \multicolumn{1}{c|}{\textbf{14386  (22.2\%)}} & \textbf{65} \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{VTR}} & \multicolumn{1}{c|}{bfly} & \multicolumn{1}{c|}{28910} & \multicolumn{1}{c|}{97} & \multicolumn{1}{c|}{26177  (9.5\%)} & \multicolumn{1}{c|}{\textbf{68}} & \multicolumn{1}{c|}{26543  (8.2\%)} & \multicolumn{1}{c|}{70} & \multicolumn{1}{c|}{25286  (12.5\%)} & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{\textbf{24975  (13.6\%)}} & \multicolumn{1}{c|}{70} & \multicolumn{1}{c|}{25277  (12.5\%)} & \multicolumn{1}{c|}{70} & \multicolumn{1}{c|}{24977  (13.6\%)} & 70 \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{dscg} & \multicolumn{1}{c|}{28252} & \multicolumn{1}{c|}{92} & \multicolumn{1}{c|}{25427  (9.9\%)} & \multicolumn{1}{c|}{67} & \multicolumn{1}{c|}{25806  (8.7\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{24595  (12.9\%)} & \multicolumn{1}{c|}{\textbf{66}} & \multicolumn{1}{c|}{\textbf{24401  (13.6\%)}} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{24764  (12.3\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{24463 (13.4\%)} & 68 \\ \cline{2-16}  

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{fir} & \multicolumn{1}{c|}{27704} & \multicolumn{1}{c|}{94} & \multicolumn{1}{c|}{24930  (10.0\%)} & \multicolumn{1}{c|}{\textbf{67}} & \multicolumn{1}{c|}{25242  (8.9\%)} & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{24112  (13.0\%)} & \multicolumn{1}{c|}{\textbf{67}} & \multicolumn{1}{c|}{23885  (13.8\%)} & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{24126  (12.9\%)} & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{\textbf{23840  (13.9\%)}} & 69 \\ \cline{2-16}

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{syn2} & \multicolumn{1}{c|}{30003} & \multicolumn{1}{c|}{93} & \multicolumn{1}{c|}{26911  (10.3\%)} & \multicolumn{1}{c|}{\textbf{67}} & \multicolumn{1}{c|}{27355  (8.8\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{26116  (13.0\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{\textbf{25901  (13.7\%)}} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{26211  (12.6\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{25950  (13.5\%)} & 68 \\ \hline

\multicolumn{1}{|c|}{\multirow{5}{*}{EPFL}} & \multicolumn{1}{c|}{div} & \multicolumn{1}{c|}{57247} & \multicolumn{1}{c|}{\textbf{4372}} & \multicolumn{1}{c|}{40889  (28.6\%)} & \multicolumn{1}{c|}{4359} & \multicolumn{1}{c|}{52336  (8.6\%)} & \multicolumn{1}{c|}{4372} & \multicolumn{1}{c|}{\textbf{40799  (28.7\%)}} & \multicolumn{1}{c|}{\textbf{4358}} & \multicolumn{1}{c|}{40881  (28.6\%)} & \multicolumn{1}{c|}{4372} & \multicolumn{1}{c|}{40880  (28.6\%)} & \multicolumn{1}{c|}{4372} & \multicolumn{1}{c|}{40840  (28.7\%)} & 4372 \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{hyp} & \multicolumn{1}{c|}{214335} & \multicolumn{1}{c|}{{24801}} & \multicolumn{1}{c|}{214240  (0.0\%)} & \multicolumn{1}{c|}{{24801}} & \multicolumn{1}{c|}{208371  (2.8\%)} & \multicolumn{1}{c|}{{24801}} & \multicolumn{1}{c|}{\textbf{205001  (4.4\%)}} & \multicolumn{1}{c|}{\textbf{24800}} & \multicolumn{1}{c|}{206527  (3.6\%)} & \multicolumn{1}{c|}{{24801}} & \multicolumn{1}{c|}{206499  (3.7\%)} & \multicolumn{1}{c|}{{24801}} & \multicolumn{1}{c|}{{206462  (3.7\%)}} & {24801} \\ \cline{2-16}

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{mem\_ctrl} & \multicolumn{1}{c|}{46836} & \multicolumn{1}{c|}{{114}} & \multicolumn{1}{c|}{46611  (0.5\%)} & \multicolumn{1}{c|}{\textbf{111}} & \multicolumn{1}{c|}{46484  (0.8\%)} & \multicolumn{1}{c|}{{114}} & \multicolumn{1}{c|}{45454  (3.0\%)} & \multicolumn{1}{c|}{\textbf{111}} & \multicolumn{1}{c|}{45342  (3.2\%)} & \multicolumn{1}{c|}{{114}} & \multicolumn{1}{c|}{45430  (3.0\%)} & \multicolumn{1}{c|}{{112}} & \multicolumn{1}{c|}{\textbf{45159  (3.6\%)}} & {112} \\ \cline{2-16}

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{sqrt} & \multicolumn{1}{c|}{24618} & \multicolumn{1}{c|}{{5058}} & \multicolumn{1}{c|}{19437  (21.0\%)} & \multicolumn{1}{c|}{{5058}} & \multicolumn{1}{c|}{21424  (13.0\%)} & \multicolumn{1}{c|}{{5058}} & \multicolumn{1}{c|}{{19217  (21.9\%)}} & \multicolumn{1}{c|}{{5058}} & \multicolumn{1}{c|}{{19219  (21.9\%)}} & \multicolumn{1}{c|}{{5058}} & \multicolumn{1}{c|}{{19217  (21.9\%)}} & \multicolumn{1}{c|}{{5058}} & \multicolumn{1}{c|}{\textbf{19215  (21.9\%)}} & \textbf{5029} \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{voter} & \multicolumn{1}{c|}{13758} & \multicolumn{1}{c|}{70} & \multicolumn{1}{c|}{10446  (24.1\%)} & \multicolumn{1}{c|}{58} & \multicolumn{1}{c|}{10155  (26.2\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{8331  (39.4\%)} & \multicolumn{1}{c|}{59} & \multicolumn{1}{c|}{8324  (39.5\%)} & \multicolumn{1}{c|}{58} & \multicolumn{1}{c|}{8328  (39.5\%)} & \multicolumn{1}{c|}{\textbf{57}} & \multicolumn{1}{c|}{\textbf{8160  (40.7\%)}} & \textbf{57} \\ \hline

\multicolumn{4}{|c|}{\textbf{Avg. Node Reduction\%}} & \multicolumn{2}{c|}{15.7\%} & \multicolumn{2}{c|}{8.9\%} & \multicolumn{2}{c|}{19.5\% (+3.8\%)} & \multicolumn{2}{c|}{19.6\% (+10.7\%)} & \multicolumn{2}{c|}{19.2\% (+3.5\%)} & \multicolumn{2}{c|}{\textbf{19.8\% (+10.9\%)}} \\ \hline
\end{tabular}%
% }
}
\caption{Detailed results of selected large size designs. Comparison of \texttt{orchestration}-substituted \texttt{O-resyn} with original \texttt{resyn}/\texttt{resyn3}.}
%\vspace{-4mm}
\label{table:resyn}
\end{table*}




% \hfill


% \begin{table*}[]
% \centering
% \resizebox{\textwidth}{!}{%
% % \subfloat[First caption]{%
% % \centering

% \begin{tabular}{|cccccccccccccccc|}
% \hline
% \multicolumn{2}{|c|}{\multirow{3}{*}{Design}} & \multicolumn{14}{c|}{AIG: \texttt{resyn}} \\ \cline{3-16} 
% \multicolumn{2}{|c|}{} & \multicolumn{2}{c|}{Baseline} & \multicolumn{2}{c|}{\texttt{resyn}} & \multicolumn{2}{c|}{\texttt{resyn3}} & \multicolumn{2}{c|}{$\widehat{\texttt{O1}}$\texttt{-resyn}} & \multicolumn{2}{c|}{$\widehat{\texttt{O1}}$\texttt{-resyn3}} & \multicolumn{2}{c|}{$\widehat{\texttt{O3}}$\texttt{-resyn}} & \multicolumn{2}{c|}{$\widehat{\texttt{O3}}$\texttt{-resyn3}} \\ \cline{3-16} 
% \multicolumn{2}{|c|}{} & \multicolumn{1}{c|}{\#Node} & \multicolumn{1}{c|}{\#Level} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Level} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Level} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Level} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Level} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \multicolumn{1}{c|}{\#Level} & \multicolumn{1}{c|}{\#Node ($\Delta$\%)} & \#Level \\ \hline
% \multicolumn{1}{|c|}{\multirow{7}{*}{ISCAS}} & \multicolumn{1}{c|}{s38584} & \multicolumn{1}{c|}{12400} & \multicolumn{1}{c|}{36} & \multicolumn{1}{c|}{10510  (15.2\%)} & \multicolumn{1}{c|}{\textbf{26}} & \multicolumn{1}{c|}{11378  (8.2\%)} & \multicolumn{1}{c|}{28} & \multicolumn{1}{c|}{10085  (18.7\%)} & \multicolumn{1}{c|}{\textbf{26}} & \multicolumn{1}{c|}{\textbf{10078  (18.7\%)}} & \multicolumn{1}{c|}{\textbf{26}} & \multicolumn{1}{c|}{\textbf{10085  (18.7\%)}} & \multicolumn{1}{c|}{\textbf{26}} & \multicolumn{1}{c|}{\textbf{10078  (18.7\%)}} & \textbf{26} \\ \cline{2-16} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{s35932} & \multicolumn{1}{c|}{11948} & \multicolumn{1}{c|}{19} & \multicolumn{1}{c|}{8598  (28.0\%)} & \multicolumn{1}{c|}{14} & \multicolumn{1}{c|}{11916  (0.3\%)} & \multicolumn{1}{c|}{19} & \multicolumn{1}{c|}{\textbf{8177  (31.6\%)}} & \multicolumn{1}{c|}{\textbf{13}} & \multicolumn{1}{c|}{\textbf{8177  (31.6\%)}} & \multicolumn{1}{c|}{\textbf{13}} & \multicolumn{1}{c|}{\textbf{8177  (31.6\%)}} & \multicolumn{1}{c|}{\textbf{13}} & \multicolumn{1}{c|}{\textbf{8177  (31.6\%)}} & \textbf{13} \\ \cline{2-16} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b17\_1} & \multicolumn{1}{c|}{27647} & \multicolumn{1}{c|}{52} & \multicolumn{1}{c|}{23096  (16.5\%)} & \multicolumn{1}{c|}{47} & \multicolumn{1}{c|}{26067  (5.7\%)} & \multicolumn{1}{c|}{47} & \multicolumn{1}{c|}{22047  (20.3\%)} & \multicolumn{1}{c|}{47} & \multicolumn{1}{c|}{\textbf{21991  (20.5\%)}} & \multicolumn{1}{c|}{47} & \multicolumn{1}{c|}{22070  (20.2\%)} & \multicolumn{1}{c|}{47} & \multicolumn{1}{c|}{22037  (20.3\%)} & 47 \\ \cline{2-16} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b18\_1} & \multicolumn{1}{c|}{79054} & \multicolumn{1}{c|}{132} & \multicolumn{1}{c|}{63826 (19.3\%)} & \multicolumn{1}{c|}{\textbf{117}} & \multicolumn{1}{c|}{70808  (10.4\%)} & \multicolumn{1}{c|}{128} & \multicolumn{1}{c|}{60232  (23.8\%)} & \multicolumn{1}{c|}{131} & \multicolumn{1}{c|}{60084  (24.0\%)} & \multicolumn{1}{c|}{131} & \multicolumn{1}{c|}{60211  (23.8\%)} & \multicolumn{1}{c|}{130} & \multicolumn{1}{c|}{\textbf{60022  (24.1\%)}} & 130 \\ \cline{2-16} 

% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b20} & \multicolumn{1}{c|}{12219} & \multicolumn{1}{c|}{66} & \multicolumn{1}{c|}{10243 (16.2\%)} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{11013  (9.9\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{9676  (20.8\%)} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{\textbf{9627  (21.2\%)}} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{9686  (20.7\%)} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{9641  (21.1\%)} & \textbf{64} \\ \cline{2-16} 

% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b21} & \multicolumn{1}{c|}{12782} & \multicolumn{1}{c|}{67} & \multicolumn{1}{c|}{10407  (18.6\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{11249  (12.0\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{9788  (23.4\%)} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{\textbf{9725  (23.9\%)}} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{9796  (23.4\%)} & \multicolumn{1}{c|}{\textbf{64}} & \multicolumn{1}{c|}{9743  (23.8\%)} & \textbf{64} \\ \cline{2-16} 

% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{b22} & \multicolumn{1}{c|}{18488} & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{15259  (17.5\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{16643  (10.0\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{14480  (21.7\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{\textbf{14399  (22.1\%)}} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{14492  (21.6\%)} & \multicolumn{1}{c|}{65} & \multicolumn{1}{c|}{14411  (22.1\%)} & 65 \\ \hline

% \multicolumn{1}{|c|}{\multirow{4}{*}{VTR}} & \multicolumn{1}{c|}{bfly} & \multicolumn{1}{c|}{28910} & \multicolumn{1}{c|}{97} & \multicolumn{1}{c|}{26389  (8.7\%)} & \multicolumn{1}{c|}{70} & \multicolumn{1}{c|}{26543  (8.2\%)} & \multicolumn{1}{c|}{70} & \multicolumn{1}{c|}{25248  (12.7\%)} & \multicolumn{1}{c|}{70} & \multicolumn{1}{c|}{\textbf{24975  (13.6\%)}} & \multicolumn{1}{c|}{70} & \multicolumn{1}{c|}{25252  (12.7\%)} & \multicolumn{1}{c|}{70} & \multicolumn{1}{c|}{25009  (13.5\%)} & 70 \\ \cline{2-16} 

% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{dscg} & \multicolumn{1}{c|}{28252} & \multicolumn{1}{c|}{92} & \multicolumn{1}{c|}{25710  (9.0\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{25806  (8.7\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{24685  (12.6\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{24401  (13.6\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{24609  (12.9\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{\textbf{24329  (13.9\%)}} & 68 \\ \cline{2-16}  

% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{fir} & \multicolumn{1}{c|}{27704} & \multicolumn{1}{c|}{94} & \multicolumn{1}{c|}{25176  (9.1\%)} & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{25242  (8.9\%)} & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{24084  (13.1\%)} & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{23885  (13.8\%)} & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{24086  (13.1\%)} & \multicolumn{1}{c|}{69} & \multicolumn{1}{c|}{\textbf{23868  (13.8\%)}} & 69 \\ \cline{2-16}

% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{syn2} & \multicolumn{1}{c|}{30003} & \multicolumn{1}{c|}{93} & \multicolumn{1}{c|}{27258  (9.1\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{27355  (8.8\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{26159  (12.8\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{25901  (13.7\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{26128  (12.9\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{\textbf{25841  (13.9\%)}} & 68 \\ \hline

% \multicolumn{1}{|c|}{\multirow{5}{*}{EPFL}} & \multicolumn{1}{c|}{div} & \multicolumn{1}{c|}{57247} & \multicolumn{1}{c|}{4372} & \multicolumn{1}{c|}{41053  (28.3\%)} & \multicolumn{1}{c|}{4372} & \multicolumn{1}{c|}{52336  (8.6\%)} & \multicolumn{1}{c|}{4372} & \multicolumn{1}{c|}{40883  (28.6\%)} & \multicolumn{1}{c|}{4372} & \multicolumn{1}{c|}{\textbf{40881  (28.6\%)}} & \multicolumn{1}{c|}{4372} & \multicolumn{1}{c|}{40909  (28.5\%)} & \multicolumn{1}{c|}{4372} & \multicolumn{1}{c|}{40908  (28.5\%)} & 4372 \\ \cline{2-16} 

% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{hyp} & \multicolumn{1}{c|}{214335} & \multicolumn{1}{c|}{24801} & \multicolumn{1}{c|}{214274  (0.0\%)} & \multicolumn{1}{c|}{24801} & \multicolumn{1}{c|}{208371  (2.8\%)} & \multicolumn{1}{c|}{24801} & \multicolumn{1}{c|}{206529  (3.6\%)} & \multicolumn{1}{c|}{24801} & \multicolumn{1}{c|}{206527  (3.6\%)} & \multicolumn{1}{c|}{24801} & \multicolumn{1}{c|}{206509  (3.7\%)} & \multicolumn{1}{c|}{24801} & \multicolumn{1}{c|}{\textbf{206507  (3.7\%)}} & 24801 \\ \cline{2-16}

% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{mem\_ctrl} & \multicolumn{1}{c|}{46836} & \multicolumn{1}{c|}{114} & \multicolumn{1}{c|}{46738  (0.2\%)} & \multicolumn{1}{c|}{114} & \multicolumn{1}{c|}{46484  (0.8\%)} & \multicolumn{1}{c|}{114} & \multicolumn{1}{c|}{45690  (2.4\%)} & \multicolumn{1}{c|}{114} & \multicolumn{1}{c|}{45342  (3.2\%)} & \multicolumn{1}{c|}{114} & \multicolumn{1}{c|}{45391  (3.1\%)} & \multicolumn{1}{c|}{114} & \multicolumn{1}{c|}{\textbf{45174  (3.5\%)}} & 114 \\ \cline{2-16}

% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{sqrt} & \multicolumn{1}{c|}{24618} & \multicolumn{1}{c|}{5058} & \multicolumn{1}{c|}{19439  (21.0\%)} & \multicolumn{1}{c|}{5058} & \multicolumn{1}{c|}{21424  (13.0\%)} & \multicolumn{1}{c|}{5058} & \multicolumn{1}{c|}{\textbf{19219  (21.9\%)}} & \multicolumn{1}{c|}{5058} & \multicolumn{1}{c|}{\textbf{19219  (21.9\%)}} & \multicolumn{1}{c|}{5058} & \multicolumn{1}{c|}{\textbf{19219  (21.9\%)}} & \multicolumn{1}{c|}{5058} & \multicolumn{1}{c|}{\textbf{19219  (21.9\%)}} & 5058 \\ \cline{2-16} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{voter} & \multicolumn{1}{c|}{13758} & \multicolumn{1}{c|}{70} & \multicolumn{1}{c|}{11033  (19.8\%)} & \multicolumn{1}{c|}{58} & \multicolumn{1}{c|}{10155  (26.2\%)} & \multicolumn{1}{c|}{68} & \multicolumn{1}{c|}{8411  (38.9\%)} & \multicolumn{1}{c|}{58} & \multicolumn{1}{c|}{8324  (39.5\%)} & \multicolumn{1}{c|}{58} & \multicolumn{1}{c|}{9231  (32.9\%)} & \multicolumn{1}{c|}{\textbf{57}} & \multicolumn{1}{c|}{\textbf{8225  (40.2\%)}} & \textbf{57} \\ \hline
% \multicolumn{4}{|c|}{\textbf{Avg. Node Reduction\%}} & \multicolumn{2}{c|}{14.8\%} & \multicolumn{2}{c|}{8.9\%} & \multicolumn{2}{c|}{19.2\% (+4.4\%)} & \multicolumn{2}{c|}{19.6\% (+10.7\%)} & \multicolumn{2}{c|}{18.8\% (+4.0\%)} & \multicolumn{2}{c|}{\textbf{19.7\% (+10.8\%)}} \\ \hline
% \end{tabular}%
% % }
% }
% \caption{Detail results of selected large designs over all benchmark suites. Comparison of \texttt{orchestration}-substituted \texttt{O-resyn} with original \texttt{resyn}/\texttt{resyn3}.}
% \vspace{-4mm}
% \label{table:resyn}
% \end{table*}




==> tbls/table_resyn_map.tex <==
\begin{table}[!htb]
\centering
% \subfloat[Second caption]{%
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|cc|cccccc|}
\hline
\multicolumn{2}{|c|}{\multirow{3}{*}{Design}} & \multicolumn{6}{c|}{Technology mapping: \texttt{resyn}} \\ \cline{3-8} 
\multicolumn{2}{|c|}{} & \multicolumn{2}{c|}{\texttt{resyn}} & \multicolumn{2}{c|}{\texttt{resyn3}} & \multicolumn{2}{c|}{Best \texttt{O-resyn}} \\ \cline{3-8} 
\multicolumn{2}{|c|}{} & \multicolumn{1}{c|}{Area} & \multicolumn{1}{c|}{Delay} & \multicolumn{1}{c|}{Area} & \multicolumn{1}{c|}{Delay} & \multicolumn{1}{c|}{Area} & Delay \\ \hline
\multicolumn{1}{|c|}{\multirow{7}{*}{ISCAS}} & s38584 & \multicolumn{1}{c|}{5955.75} & \multicolumn{1}{c|}{12.0} & \multicolumn{1}{c|}{6129.26} & \multicolumn{1}{c|}{\bf 11.0} & \multicolumn{1}{c|}{\textbf{5747.79}} & 12.0 \\ \cline{2-8} 
\multicolumn{1}{|c|}{} & s35932 & \multicolumn{1}{c|}{\textbf{5282.22}} & \multicolumn{1}{c|}{\bf 5.0} & \multicolumn{1}{c|}{6193.42} & \multicolumn{1}{c|}{6.0} & \multicolumn{1}{c|}{5414.85} & {\bf 5.0} \\ \cline{2-8} 
\multicolumn{1}{|c|}{} & b17\_1 & \multicolumn{1}{c|}{12981.71} & \multicolumn{1}{c|}{18.0} & \multicolumn{1}{c|}{14354.19} & \multicolumn{1}{c|}{\bf 17.0} & \multicolumn{1}{c|}{\textbf{12952.42}} & {\bf 17.0} \\ \cline{2-8} 
\multicolumn{1}{|c|}{} & b18\_1 & \multicolumn{1}{c|}{36892.34} & \multicolumn{1}{c|}{\bf 54.0} & \multicolumn{1}{c|}{39672.16} & \multicolumn{1}{c|}{58.0} & \multicolumn{1}{c|}{\textbf{36264.68}} & 56.0 \\ \cline{2-8} 

\multicolumn{1}{|c|}{} & b20 & \multicolumn{1}{c|}{5013.41} & \multicolumn{1}{c|}{25.0} & \multicolumn{1}{c|}{5117.39} & \multicolumn{1}{c|}{\bf 24.0} & \multicolumn{1}{c|}{\textbf{4718.43}} & {\bf 24.0} \\ \cline{2-8}

\multicolumn{1}{|c|}{} & b21 & \multicolumn{1}{c|}{5154.01} & \multicolumn{1}{c|}{25.0} & \multicolumn{1}{c|}{5289.59} & \multicolumn{1}{c|}{\bf 24.0} & \multicolumn{1}{c|}{\textbf{4877.81}} & {\bf 24.0} \\ \cline{2-8}

\multicolumn{1}{|c|}{} & b22 & \multicolumn{1}{c|}{7464.92} & \multicolumn{1}{c|}{\bf 25.0} & \multicolumn{1}{c|}{7646.79} & \multicolumn{1}{c|}{\bf 25.0} & \multicolumn{1}{c|}{\textbf{7251.37}} & {\bf 25.0} \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{VTR}} & bfly & \multicolumn{1}{c|}{15804.08} & \multicolumn{1}{c|}{\bf 28.0} & \multicolumn{1}{c|}{15589.98} & \multicolumn{1}{c|}{\bf 28.0} & \multicolumn{1}{c|}{\textbf{14869.39}} & 29.0 \\ \cline{2-8}

\multicolumn{1}{|c|}{} & dscg & \multicolumn{1}{c|}{15378.06} & \multicolumn{1}{c|}{\bf 28.0} & \multicolumn{1}{c|}{15475.00} & \multicolumn{1}{c|}{\bf 28.0} & \multicolumn{1}{c|}{\textbf{14846.70}} & {\bf 28.0} \\ \cline{2-8}

\multicolumn{1}{|c|}{} & fir & \multicolumn{1}{c|}{15709.50} & \multicolumn{1}{c|}{\bf 27.0} & \multicolumn{1}{c|}{15544.94} & \multicolumn{1}{c|}{28.0} & \multicolumn{1}{c|}{\textbf{14794.36}} & 28.0 \\ \cline{2-8}

\multicolumn{1}{|c|}{} & syn2 & \multicolumn{1}{c|}{15943.05} & \multicolumn{1}{c|}{28.0} & \multicolumn{1}{c|}{15904.37} & \multicolumn{1}{c|}{28.0} & \multicolumn{1}{c|}{\textbf{15289.84}} & {\bf 27.0} \\ \hline

\multicolumn{1}{|c|}{\multirow{5}{*}{EPFL}} & div & \multicolumn{1}{c|}{23828.21} & \multicolumn{1}{c|}{1452.0} & \multicolumn{1}{c|}{\textbf{19881.61}} & \multicolumn{1}{c|}{1471.0} & \multicolumn{1}{c|}{24884.07} & {\bf 1435.0} \\ \cline{2-8} 

\multicolumn{1}{|c|}{} & hyp & \multicolumn{1}{c|}{159726.43} & \multicolumn{1}{c|}{\bf 8315.0} & \multicolumn{1}{c|}{159690.55} & \multicolumn{1}{c|}{8316.0} & \multicolumn{1}{c|}{\textbf{159446.83}} & {\bf 8315.0} \\ \cline{2-8}

\multicolumn{1}{|c|}{} & mem\_ctrl & \multicolumn{1}{c|}{13098.80} & \multicolumn{1}{c|}{\bf 37.0} & \multicolumn{1}{c|}{12937.87} & \multicolumn{1}{c|}{\bf 37.0} & \multicolumn{1}{c|}{\textbf{12616.00}} & {\bf 37.0} \\ \cline{2-8}

\multicolumn{1}{|c|}{} & sqrt & \multicolumn{1}{c|}{10913.79} & \multicolumn{1}{c|}{\bf 2003.0} & \multicolumn{1}{c|}{\textbf{10069.77}} & \multicolumn{1}{c|}{2018.0} & \multicolumn{1}{c|}{10218.57} & {\bf 2003.0} \\ \cline{2-8} 

\multicolumn{1}{|c|}{} & voter & \multicolumn{1}{c|}{8692.15} & \multicolumn{1}{c|}{28.0} & \multicolumn{1}{c|}{7747.81} & \multicolumn{1}{c|}{29.0} & \multicolumn{1}{c|}{\textbf{7061.83}} & {\bf 26.0} \\ \hline
\multicolumn{2}{|c|}{\textbf{Avg. Area Reduction\%}} & \multicolumn{2}{c|}{\color{red}-4.2\%} & \multicolumn{2}{c|}{\color{red}-4.5\%} & \multicolumn{2}{c|}{ - } \\ \hline
\end{tabular}%
% }
}
\caption{Detailed results of selected large size designs. Comparison of technology mapping of \texttt{resyn}/\texttt{resyn3} with Best \texttt{O-resyn}. Area and delay are reported in $um^2$ and $ps$.}
\vspace{-4mm}
\label{table:resyn_map}
\end{table}

==> tbls/table_runtime.tex <==
\begin{table}[!htb]
\centering
\footnotesize
% \subfloat[Second caption]{%
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|cc|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\multirow{3}{*}{Design}} & \multicolumn{4}{c|}{AIG} \\ \cline{3-6}
\multicolumn{2}{|c|}{} & \texttt{rw} & \texttt{rs} & \texttt{rf} & Ours \\ \cline{3-6} 
\multicolumn{2}{|c|}{} & \#Iteration & \#Iteration & \#Iteration & \#Iteration \\ \hline
\multicolumn{1}{|c|}{\multirow{7}{*}{ISCAS}} & s38584 & 12396 & 12277 & 12278 & \textbf{1489} \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & s35932 & 11948 & 11948 & 11948 & \textbf{2014} \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & b17\_1 & 27518 & 27504 & 27611 & \textbf{3635} \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & b18\_1 & 78440 & 78485 & 78891 & \textbf{10274} \\ \cline{2-6}
\multicolumn{1}{|c|}{} & {b20} & 12093 & 12092 & 12094 & \textbf{1259} \\ \cline{2-6} 
\multicolumn{1}{|c|}{} & b21 & 12498 & 12525 & 12658 &  \textbf{1402}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & {b22} & 18151 & 18140 & 18418 &  \textbf{2109}\\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{VTR}} & bfly & 28904 & 28895 & 28910 &  \textbf{2340}\\ \cline{2-6} 
\multicolumn{1}{|c|}{} & {dscg} & 28237 & 28238 & 28250 &  \textbf{2304}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & fir & 27689 & 27686 & 27703 &  \textbf{2357}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & {syn2} & 29991 & 29990 & 30003 &  \textbf{2318}\\ \hline
\multicolumn{1}{|c|}{\multirow{5}{*}{EPFL}} & {div} & 57245 & 57239 & 57235 &  \textbf{16122}\\ \cline{2-6} 
\multicolumn{1}{|c|}{} & {hyp} & 214335 & 214335 & 214335 &  \textbf{7113}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & mem\_ctrl & 46836 & 46836 & 46836 &  \textbf{2602}\\ \cline{2-6}
\multicolumn{1}{|c|}{} & sqrt & 24618 & 24617 & 24617 &  \textbf{5290}\\ \cline{2-6} 
\multicolumn{1}{|c|}{} & voter & 13697 & 13753 & 13758 & \textbf{3712} \\ \hline
\end{tabular}
% }
}
\caption{Complexity evaluation in iteration count with selected large size designs.}
%\vspace{-4mm}
\label{table:it_count}
\end{table}
